Self-learning for weakly supervised Gleason grading of local patterns

Prostate cancer is one of the main diseases affecting men worldwide. The gold standard for diagnosis and prognosis is the Gleason grading system. In this process, pathologists manually analyze prostate histology slides under microscope, in a high time-consuming and subjective task. In the last years, computer-aided-diagnosis (CAD) systems have emerged as a promising tool that could support pathologists in the daily clinical practice. Nevertheless, these systems are usually trained using tedious and prone-to-error pixel-level annotations of Gleason grades in the tissue. To alleviate the need of manual pixel-wise labeling, just a handful of works have been presented in the literature. Motivated by this, we propose a novel weakly-supervised deep-learning model, based on self-learning CNNs, that leverages only the global Gleason score of gigapixel whole slide images during training to accurately perform both, grading of patch-level patterns and biopsy-level scoring. To evaluate the performance of the proposed method, we perform extensive experiments on three different external datasets for the patch-level Gleason grading, and on two different test sets for global Grade Group prediction. We empirically demonstrate that our approach outperforms its supervised counterpart on patch-level Gleason grading by a large margin, as well as state-of-the-art methods on global biopsy-level scoring. Particularly, the proposed model brings an average improvement on the Cohen's quadratic kappa (k) score of nearly 18% compared to full-supervision for the patch-level Gleason grading task.

==> backup/00_Abstract_Backup.tex <==
\begin{abstract}

Prostate cancer is one of the main diseases affecting men worldwide. The gold standard for diagnosis and prognosis is the Gleason grading system. In this process, pathologists manually analyze prostate histology slides under microscope, in a high time-consuming and subjective task. In the last years, computer-aided-diagnosis (CAD) systems have emerged as a promising tool that could support pathologists in the daily clinical practice. These systems are usually trained using tedious and prone-to-error pixel-level annotations of Gleason grades in the tissue. Few works have proposed the use of biopsy-level Gleason score to avoid the tedious process of manual data labeling. Although these works reach promising results for global scoring, the location of cancerous patterns in the tissue is only qualitatively addressed. Accurate heatmaps highlighting the cancerous regions that the system is focusing on are crucial to the reliability of CAD systems. They provide explainability to the system's output and give confidence to pathologist that the model is focusing on medical relevant features. In this work, we propose a weakly-supervised deep-learning system based on self-learning CNNs able to accurately perform both, grading of patch-level patterns and biopsy-level scoring using only the global Gleason score of gigapixel whole slide images during training. Using this model, we obtained an average Cohen's quadratic kappa ($\kappa$) of $0.82$ for the patch-level Gleason grading on three different external datasets and an average $\kappa$ of $0.84$ on two different test sets for global Grade Group prediction. In the experimental stage, we performed an extensive comparison of the proposed approach with state-of-the-art supervised methods on the same test subsets. The self-learning CNN pipeline outperforms supervised methods trained using pixel-level annotations thanks to the absence of the annotator's bias and the capability of using large datasets during training. Regarding the global biopsy-level scoring, using raw features obtained from the patch-level classifier showed to generalize better the subjective global scoring than previous approaches in the literature. 


\end{abstract}

==> backup/01_Introduction_Backup.tex <==
\section{Introduction}
\label{sec:introduction}

% ------------
%% Motivation

% Prostate cancer and Gleason

Prostate cancer is one of the major diseases affecting men worldwide. It accounts for $14.5\%$ of all cancers in men \cite{wcrf} and, according to the World Health Organization, its yearly incidence will increase to 1.8 million cases this decade \cite{who}. The Gleason grading system \cite{gleason} is the main tool for its diagnosis and prognosis. This system describes different stages of cancer based on the morphology and distribution of glands in prostate biopsies. Specifically, the Gleason (GG) grades observable in histology samples range from $3$ (GG3) to $5$ (GG5). Fig. \ref{fig1} shows representative patterns of each grade

\begin{figure}[htb]
\captionsetup[subfloat]{farskip=1pt,captionskip=0.8pt}
    \centering
      \subfloat[\label{fig1a}]{\includegraphics[width=.235\linewidth, frame]{Figures/examples_introduction/NC.jpg}}
      \hspace*{\fill}
      \subfloat[\label{fig1b}]{\includegraphics[width=.235\linewidth, frame]{Figures/examples_introduction/gg3.jpg}}
      \hspace*{\fill}
      \subfloat[\label{fig1c}]{\includegraphics[width=.235\linewidth, frame]{Figures/examples_introduction/gg4.jpg}}
      \hspace*{\fill}
      \subfloat[\label{fig1d}]{\includegraphics[width=.235\linewidth, frame]{Figures/examples_introduction/gg5.jpg}}
    \caption{Histology regions of prostate biopsies. (a): region containing benign glands, (b): region containing GG3 glandular structures, (c): region containing GG4 patterns, (d): region containing GG5 patterns. GG: Gleason grade.}
    \label{fig1}
\end{figure}

% Clinical procedure and limitations
In order to make a diagnosis of prostate cancer, pathologists extract small portions of tissue, which are laminated and stained using Hematoxylin and Eosin. Then, the slides are carefully analyzed under the microscope to grade local glandular patterns according the Gleason grading system. Finally, the two most prominent grades in terms of proportion and severity are used to obtain a global Gleason score as prognosis marker. For instance, the Gleason score $3+5=8$ would be assigned to a sample in which the main cancerous Gleason grade is GG3 and the second is GG5. Recently, after the $2014$ conference of the International Society of Urological Pathology, a new grading system denominated Grade Group \cite{Epstein2015ASystem} is being used. This systems takes into account the  different prognosis between patients with Gleason score $3+4=7$ and $4+3=7$, including them to different groups (Grade Group $2$ and $3$, respectively). The previously described process of histology prostate biopsy analysis is characterized by high time consumption and large intra and inter pathologist variability \cite{Burchardt2008InterobserverMicroarrays}.


% CAD systems using annotations limitations
Computer-aided diagnosis (CAD) systems based on computer vision algorithms are able to support pathologists in the daily analysis of prostate biopsies. However, the development of these applications is limited due to the high data-demanding character of deep learning algorithms, the large size of digitized biopsies (denominated whole slide images) and the difficulty in obtaining pixel-level labeled histology images \cite{Komura2018MachineAnalysis}. CAD systems are usually developed classifying local cancerous regions, which are finally combined into a global score. In the case of prostate cancer, this requires manual annotation using multi-resolution graphical user interfaces to accurately delimit the cancerous structures using the Gleason grading system. This is a laborious, time-consuming process prone to error due to pathologists discouragement. Moreover, heterogeneous epithelial cancer such as prostate one require a large number of samples to cover the wide range of possible patterns, which is difficult to reach on annotated datasets.    

% CAD systems using weak supervision limitations: importance of heatmaps
The limitations of using annotated datasets has encouraged the development of weakly-supervised methods able to utilize global labels during the training process. In the last years, few works in the literature have proposed the use of the global Gleason score (easily accessible from the clinical record) to develop CAD systems for prostate biopsy scoring (these works are detailed in Section \ref{ssec:rw2}). The main limitations of the proposed approaches is that they focus on the global-level scoring, while the challenge of local grading cancerous patterns is only qualitatively validated or not addressed. The classification of local Gleason grades in prostate biopsies is the basis of a explainable prostate CAD system. The resultant heatmaps support the biopsy-level scoring provided by the system, and they demonstrate that the model relies on relevant medical markers. Thus, the accuracy of the proposed methods in this task should be validated, in order to provide confidence to pathologists in the daily-use of the CAD system. 


% -----------------------
%% Objective and Novelties

In this work, we propose a weakly-supervised deep-learning framework based on self-learning convolutional neural networks able to perform both, the global scoring of biopsies and the local grading of cancerous structures in the tissue using the global Gleason score during training. To the best of authors's knowledge, this is the first work in the literature aiming for accurately grading local cancerous patterns in prostate whole slide images using biopsy-level labels. In the following lines, we summarize the main contributions of this paper. We propose an end-to-end CNN architecture based on patch-level inference aggregation able to detect high-confidence cancerous instances in a weakly-supervised Multiple-Instance Learning (MIL) task training with biopsy-level labels. Then, we propose a self-learning framework that converts the MIL dataset into a pseudo-supervised task, using the patches predicted by the previous model and a post-processing label refinement. During the experimental stage, we demonstrate that weakly-supervised models trained on large data sets are able to generalize better for the patch-level Gleason grading than supervised models trained in smaller databases with pixel-level annotations. Finally, we predict the global biopsy-level score based on the aggregation of local features using the models trained for the patch-level Gleason grading.


% -----------------------
%% Organization

The remainder of this paper is divided into five sections. First, Section \ref{sec:relWork} describes related works in the literature, in terms of self-learning methods (Section \ref{ssec:rw1}) and the analysis of prostate histology samples (Section \ref{ssec:rw2}). Then, Section \ref{sec:dataset} describes the four different datasets used to develop and validate the proposed methodology. Section \ref{sec:methods} details these methods. Concretely, Section \ref{ssec:meth1} and \ref{ssec:meth2} describe the self-learning CNN pipeline for patch-level Gleason grading using weak global labels. Section \ref{ssec:meth1} exposes the novel Teacher CNN architecture that performs patch-level classification using biopsy-level labels during training, and Section \ref{ssec:meth2} explains the label distillation process carried out to train Student model. Section \ref{ssec:meth3} details the method proposed for global scoring of biopsies, based on the features extracted by the patch-level classifier. All these methods are validated during the experimental stage, described in detail in Section \ref{sec:experiments}. Finally, the conclusions and future directions extracted from our work are summarized in Section \ref{sec:conclusions}.

==> backup/02_Related_Work_Backup.tex <==
\section{Related Work}
\label{sec:relWork}

% --------------------------------
%% Self-Learning CNNs
\subsection{Self-Learning CNNs}
\label{ssec:rw1}

Self-learning (a.k.a. self-paced learning or self-training) is a training procedure introduced in \cite{Scudder1965ProbabilityMachines} that aims to use the knowledge of a firstly trained model (usually called Teacher) into a second model (known as Student). Interest in this technique has grown in recent years due to the promising results obtained in semi- and weakly-supervised learning. The knowledge used from Teacher model varies on each application. For instance, in semi-supervised learning, Teacher is used to obtain pseudo-labels from non-labeled data \cite{Chen2020BigLearners,Xie2019Self-trainingClassification,Yalniz2019Billion-scaleClassification, Veit2017LearningSupervision}. Also, different works in weakly-supervised object localization use Teacher model to select regions of interest from the image to train Student model in a simplified dataset \cite{Bazzani2016Self-taughtNetworks, Sangineto2019SelfDetection, Jie2017DeepLocalization}. 

Inspired by these previous works, we adapt the self-learning concept to the Multiple Instance Learning framework using clusters of patches from whole slide images, in order to accurate classify instances using bag-level labels during training.

% --------------------------------
%% Gleason grading in Prostate Histology Images
\subsection{Gleason Grading in Prostate Histology Images}
\label{ssec:rw2}

A reliable Computer-Aided Diagnosis system in prostate cancer using histology biopsies aim two main tasks: the global scoring of slides and the quantification and localization of cancerous tissue, both using the Gleason grading system. Due to the large dimension of whole slide images and the computational limitations of CNNs, the basis of these systems is the use of small patches extracted from the slide. The proposed methods in the literature can be divided into two categories: bottom-up frameworks, which perform a patch-level classification of Gleason grades using pathologists annotation, and top-down methods, which perform a pseudo-labeling of the patches based on the global Gleason score of the sample. 

First works in this field focused on bottom-up frameworks. They usually fine-tune well-known CNN architectures in a supervised patch-level classification. Note that these methods require pixel-level expert annotations to obtain the ground truth. Nir et al. \cite{Nir2018AutomaticExperts,Nir2019ComparisonImages} obtained a patch-level Cohen's quadratic kappa ($\kappa$) of $0.60$ in the validation set, and Arvaniti et al. \cite{Arvaniti2018AutomatedLearning} and Silva et al. \cite{Silva-rodriguez2020GoingR} reached $0.55$ and $0.77$ in their respective test set. In the last work, Silva et al. tested their model on two external subsets, annotated by different pathologists. The results showed a decrease in the performance ($\kappa=0.64$ and $\kappa=0.51$), which calls into question the generalization capability of supervised models trained on reduced datasets.

Lately, different works in the literature have proposed approaches in order to overcome the need of pixel-level annotations of Gleason grades. These methods are based in a top-down strategy, where global labels (easily accessible from the patient clinical record) are assigned to local regions of interest, to train a weakly-supervised patch-level classification model using pseudo-labels. In this line, Campanella et al. \cite{Campanella2019Clinical-gradeImages} assigned the global label (cancerous against non-cancerous) to all the patches of the slide. Jiménez del Toro et al. \cite{JimenezdelToro2017ConvolutionalScore} and Otálora et al. \cite{Otalora2019StainingPathology} used color-based filtering to select only patches with high presence of nuclei in cancerous slides, and Ström et al. \cite{Strom2020ArtificialStudy} followed a similar strategy using Laplacian filters. Bulten et al. \cite{Bulten2020AutomatedStudy} proposed a semi-supervised pipeline, and discarded patches that presented low amount of epithelial tissue. In that work, glandular tissue was previously segmented using an UNet trained using pixel-level annotations. Although these works provided promising results for the global biopsy-level scoring (which are detailed in the next paragraph), the patch-level classification was not quantitatively validated. Few works only performed a qualitative evaluation of the produced heatmaps. In these methods, the localization of Gleason grades in the tissue could be affected by the assumptions made to obtain the patch-level pseudo-labels. Accurate localization of Gleason grades in the tissue is a major task that CAD systems should address. The produced heatmaps provide explainability to the system, and ensures that the output is based on medical factors to entrust pathologists in their daily use.  

Regarding the global scoring of biopsies, the main approach is based on aggregating the patch-level predictions of Gleason grades via the percentage of each grade in the tissue. Different models have been proposed to predict the global Gleason score or ISUP group. Arvaniti et al. and Bulten et al. assigned the primary and secondary grades above certain threshold of tissue, obtaining a $\kappa$ of $0.75$ to predict the Gleason score and a $\kappa$ of $0.85$ to predict the Grade Group, respectively. Nagpal et al. \cite{Nagpal2019DevelopmentCancer} trained a k-nearest neighbor model to predict the Grade Group, reaching an accuracy of $0.70$. Silva et al. proposed the use of a multilayer perceptron to predict the Gleason score, archieving a $\kappa$ of $0.82$ on the test cohort. Also, Ström et al. proposed the use of random forest algorithm and reached a $\kappa$ of $0.84$. Most of the CAD systems reach promising results, at the level of inter-pathologists agreement, quantified at $\kappa = 0.71$ by Arvaniti et al., at $\kappa = 0.73$ by Ström et al. \cite{Strom2020ArtificialStudy} and at $\kappa = 0.81$ by Bulten et al.





==> backup/03_Dataset_Backup.tex <==
\section{Dataset}
\label{sec:dataset}

The experiments described in this paper are conducted using several public datasets well known in the prostate cancer histology literature. Concretely, two different datasets of prostate whole slide images are used to validate the global biopsy-level methodology, while three databases with pixel-level annotations are used to test the local Gleason grading capability of the proposed methods.

Regarding the datasets used to validate the biopsy-level performance, the recently released database from PANDA challenge \cite{wouter_bulten_2020_3715938}, competition of the MICCAI 2020 conference, is used to train the proposed algorithms and to test them. This set consist of $10,415$ prostate whole slide images whose primary and secondary Gleason grades have been labelled by expert pathologists. The gigapixel images were resampled to $10\times$ resolution, and randomly clustered to three groups for training, validating and testing. Also, in order to test the models, the external SICAP database presented in \cite{Silva-rodriguez2020GoingR} is used. This dataset consist of 155 prostate whole slide images with both global primary and secondary Gleason grades annotated by expert pathologists. The obtained partition in PANDA set and the Gleason score distribution for each dataset are presented in Table \ref{tab:dataWSI}.

% Table with wsi database:
\begin{table}[htb]

    \centering
    \caption{Datasets of prostate biopsies used. Whole slide images partition and Gleason scores (GS) distribution.}
    \label{tab:dataWSI}

    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\textbf{Partition}} & \textbf{NC} & \textbf{GS6} & \textbf{GS7} &  \textbf{GS8} &  \textbf{GS9} &  \textbf{GS10}\\
    \hline
    \hline
    \multicolumn{7}{c}{PANDA} \\
    \hline
    \hline
    Train & $2297$ & $2122$ & $2075$ & $1002$ & $874$ & $99$\\
    \hline
    Validation & $98$ & $89$ & $85$ & $42$ & $33$ & $6$\\
    \hline
    Test & $497$ & $455$ & $425$ & $205$ & $190$ & $22$\\
    \hline
    Total & $2892$ & $2666$ & $2585$ & $1249$ & $1097$ & $127$\\
    \hline
    \hline
    \multicolumn{7}{c}{SICAP} \\
    \hline
    \hline
    Test & $36$ & $14$ & $45$ & $18$ & $35$ & $7$\\
    \hline
    \end{tabular}

\end{table}

In order to validate the capability of  the proposed methods to grade local cancerous patterns, three different external datasets containing pixel-level annotations of Gleason grades are used. Concretely, the test cohort from SICAP dataset and the ARVANITI \cite{Arvaniti2018AutomatedLearning} and GERYTCH \cite{Gertych2015MachineProstatectomies} databases are used. For these sets, patches of size $512^2$ pixels are extracted at $10\times$ resolution. The patch-level labels are assigned by majority voting of the pixel-level annotations, and the non-cancerous class is assigned to patches containing only benign annotations. The number of patches from each dataset and the Gleason grade distribution is presented in Table \ref{tab:dataPatches}.

% Table with wsi SICAP database:
\begin{table}[htb]

    \centering
    \caption{Datasets with patch-level Gleason grade annotations used for testing. Distribution of the patches among non-cancerous (NC) and the different Gleason grades (GG).}
    \label{tab:dataPatches}

    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\textbf{Database}} & \textbf{NC} & \textbf{GG3} & \textbf{GG4} &  \textbf{GG5}\\
    \hline
    
    SICAP & $644$ & $393$ & $853$ & $232$\\
    \hline
    ARVANITI & $115$ & $274$ & $210$ & $104$\\
    \hline
    GERYTCH & $32$ & $95$ & $216$ & $70$\\
    \hline
    \end{tabular}

\end{table}

The three external databases were normalized to homogenize the color distribution to the PANDA database. Concretely, the method presented in \cite{Vahadane2015Structure-preservedImages} was used after applying a channel-wise histogram matching to the images from the external databases to a PANDA reference image. This image was selected by the pathologists involved in this work based on its structural and stain properties.


==> backup/04_Methods_Backup.tex <==
\section{Methods}
\label{sec:methods}

The methodological core of this work is a self-supervised trained CNN classifier able to grade prostate histology patches using only the biopsy-level Gleason score during training. The proposed workflow is presented in Fig. \ref{figselfLear}.

\begin{figure*}[htb]
    \begin{center}
    \includegraphics[width=.99\textwidth]{Figures/self_training.pdf}
    \caption{Self-learning CNNs pipeline for weakly supervised Gleason grading of local cancerous patterns in whole slide images. MIL: multiple-instance learning; WSI: whole slide image; NC: non-cancerous; GS: Gleason score; GG: Gleason grade.}
    \label{figselfLear}
    \end{center}
\end{figure*}

In the context of multiple-instance learning (MIL), a prostate biopsy is considered as a bag $X_{b}$ containing instances $x_{b,i}$. The instances, or patches, are extracted from the slides using a moving-window of $512$ pixels and stride of $256$. A tissue mask is obtained from the slide by Otsu's thresholding, and patches with less than $20\%$ of tissue are discarded.

In this work, we address the problem of predicting the instance-level labels $y_{b,i}$ via a weakly-supervised training, where only the biopsy-level label $Y_{b}$ is known. $Y_{b}$ is obtained using the primary and secondary Gleason grades of the biopsy indicated in the Gleason score. Concretely, the non-cancerous (NC), Gleason grade (GG) $3$, $4$ and $5$ classes are included in $Y_{b}$ as a multi-label one-hot-encoding ground truth.

The self-supervised framework is composed by two CNNs: Teacher ($\theta^t$) and Student ($\theta^s$). The first model classifies high-confidence patches in a noisy MIL framework, and the second uses the instance-level pseudo-labels based on Teacher model predictions for training on a pseudo-supervised dataset. 

% --------------------------------
%% Teacher model

\subsection{Teacher Model}
\label{ssec:meth1}

Teacher model aims to grade high-confidence patches using biopsy-level labels for learning. Thus, the training process is based on the global Gleason grade prediction ($\tilde{Y}^{t}_{b}$) from the instances ($x_{b,i}$) such that:

\begin{equation}
\label{eq:tm1}
\tilde{Y}^{t}_{b} = f(\{x_{b,1},...,x_{b,i},...,x_{b,I}\},\theta^t)
\end{equation}

\noindent where $I$ denotes the total number of patches in the slide and $\theta$ the model weights.

To accomplish the inference of instance-level predictions, the learning process is based on the aggregation of patch-level predictions. Thus, Teacher model predicts the Gleason grade instances $y$ such that:

\begin{equation}
\label{eq:tm2}
\tilde{y}^t_{b,i} = f(x_{b,i},\theta^t)
\end{equation}

Teacher model takes tiles of size $256\times256$ as input, and uses VGG16 architecture as backbone with weights pre-trained on Imagenet for the feature extraction stage. Then, a global-average pooling and a dense layer with soft-max activation is used as top model.

Then, the aggregation function $p(\cdot)$ resumes all the instance-level predictions into one representative value that serves as global-level inference as follows:

\begin{equation}
\label{eq:tm3}
\tilde{Y}^{t}_{b} = p(\{\tilde{y}^t_{b,1},...,\tilde{y}^t_{b,i},...,\tilde{y}^t_{b,I}\})
\end{equation}

The pooling function should be robust to the MIL characteristics. A bag-level class could be positive if just one of the instances is positive for that class. For instance, the use of average pooling would diminish the global cancerous classes activation if the slide contains a large number of non-cancerous patches. Inspired by the properties observed in the max-pooling operation in weakly-supervised segmentation tasks \cite{Oquab2012IsFree}, we propose the use of a slide-level max-pooling. Using this operation, the global probability per class is the maximum of the patch-level inferences.

Finally, multi-label binary-cross entropy loss is used during training for gradient estimation. Concretely, the loss is obtained using only the cancerous grades under the assumption that all slides could contain non-cancerous regions, but only cancerous slides contain patches with Gleason patterns.

A summary of the Teacher model training is illustrated in Fig. \ref{figteacherModel}. 

\begin{figure}[H]
    \begin{center}
    \includegraphics[width=.5\textwidth]{Figures/cnn_aggregation.pdf}
    \caption{Teacher CNN for the prediction of local Gleason grades in a Multiple-Instance Learning framework. GG: Gleason grade.}
   \label{figteacherModel}
    \end{center}
\end{figure}

\textbf{Implementation Details} -- The proposed Teacher model is based on the aggregation of patch-level outputs (Gleason grade predictions). Due to the variable amount of instances in a biopsy $I$, the architecture cannot be trained using a mini-batch strategy. Thus, the learning process is carried out using a batch size of $1$ slide. The number of patches vary from $40$ up to $300$ in the training set. In order to avoid computational limitations, up to $200$ random patches are used in each iteration.

% --------------------------------
%% Student model

\subsection{Student Model}
\label{ssec:meth2}

Student model aims to perform a patch-level Gleason grade prediction based on a pseudo-supervised data set of images, using pseudo-labels based on Teacher model predictions.

First, all instances from the dataset are predicted using the Teacher model. Then, a label refinement process is carried out based on patch-level Teacher model predictions ($\tilde{y}^{t}_{b,i}$) and the known global slide-level labels ($Y_{b}$). In this process, labels are modified, and patches are discarded under the following premises:

\begin{equation}
    \label{eq:MIL}
       \hat{y}{^t}_{b,i}=
       \begin{cases} 
        NC, & \text{if}\ G \not\subset Y_{b} \\ 
        G, & \text{if}\ G \subset \tilde{y}{^t}_{b,i} \land G \subset Y_{b} \\
        \text{Discarded}, & \text{Otherwise}
        \end{cases}
\end{equation}
\noindent where $NC$ denotes the non-cancerous class, $G$ an undefined Gleason grade, and $\tilde{y}^{t}_{b,i}$ is the hard one-hot encoding of the Teacher model prediction for certain patch $i$, belonging to the slide $b$.

Thus, only the patches classified as certain Gleason grade that belongs to a slide containing that grade are kept for Student model learning. Regarding the non-cancerous patches, those are obtained only from known benign slides. This label refinement post-processing, together with the simplification of the problem from a MIL to a pseudo-supervised framework, allows Student model to better learning feature representations of the patches.

Finally, a model with the same architecture as Teacher model is trained minimizing the categorical-cross entropy between predictions and pseudo-labels. Class weights are applied in the loss function to deal with class unbalance such that:

\begin{equation}
\label{eq:loss}
L(\tilde{y}^s_{b,i},\tilde{y}^t_{b,i}) = - \frac{1}{C}\sum_{c=1}^{C}w_{c}(\hat{y}^t_{b,i,c}log(\tilde{y}^s_{b,i,c}))
\end{equation}

\noindent where $c$ indicates each of the $C$ classes (i.e. non-cancerous, Gleason grade $3$, $4$ and $5$). $w_{c}= (C \times N) / N_{c}$ is the weight applied to each class, being $N$ the total number of images and $N_{c}$ the number of images belonging to class $c$.

%Once Student model is trained, the resultant model becomes Teacher model, and the pseudo-labeling process of the images is repeated to train a new Student model from scratch. This process is repeated $T$ times, until no more instances are added to the pseudo-supervised set.

% --------------------------------
%% Global Gleason scoring

\subsection{Biopsy-Level Gleason Scoring}
\label{ssec:meth3}

Once the Gleason grades are located in the tissue using the previously presented self-learning CNN, we propose the use of the specialized features extracted by Student model to predict the global Gleason score.

Thus, being $z{^s}_{b,i}$ the features extracted by Student model to each patch after the global-average pooling layer (see Section \ref{ssec:meth1}), the slide-level feature representation is obtained by global averaging of the instance-level features as follows:

\begin{equation}
\label{eq:globalscoring}
z^{s}_{b} = \frac{1}{I} \sum_{i} z^{s}_{b,i}
\end{equation}

Then, two different models are used to predict both the global Gleason score and Grade Group. First, a neural-network-based multi-layer perceptron ($MLP$) composed of one hidden layer with 64 neurons and ReLU activation is used to predict the one-hot-encoding of the global labels. In this case, soft-max activation is used in the output layer and the weights are optimized using categorical cross-entropy loss. Secondly, a k-Nearest Neighbors ($kNN$) model is used to compare the generalization capability of neural networks and non-parametric models for this task. 

%Then, a dense layer $w$ with soft-max activation is trained to predict the global biopsy-label such that $\tilde{Y}^{t}_{b} = w * z^{s}_{b}$. The weights are updated using the categorical cross entropy loss against the reference labels ${Y}^{t}_{b}$. Note that in this case, the reference is the one-hot-encoding of the Gleason score or Grade Group.

==> backup/05_Experiments_Results_Backup.tex <==
\section{Experiments and Results}
\label{sec:experiments}

In this section, we describe the experiments carried out to validate the proposed methods for both tasks: grading of local patterns (Section \ref{ssec:exp2}) and global scoring of biopsies (Section \ref{ssec:exp3}). The results obtained using the different externals datasets presented in Section \ref{sec:dataset} are exposed. We also perform an extensive comparison with previous results obtained in the same test subsets in \cite{Silva-rodriguez2020GoingR}. In that work (we refer later to it as $Supervised$), a supervised model is trained using pixel-level annotations of Gleason grades performed by expert pathologists on whole slide images from SICAP database (see Section \ref{sec:dataset} for a detailed description of the dataset). In order to evaluate the different approaches, the metrics used are accuracy (ACC), f1-score (F1S) per class and its average, and Cohen's quadratic kappa ($\kappa$) \cite{Cohen1968WeightedCredit}. The last metric, $\kappa$, is the main figure of merit used in prostate Gleason grading. It takes into account that the Gleason system consist on a set of ordered classes, and error between adjacent classes should be less penalized.

% --------------------------------
%% Local Gleason grading

\subsection{Grading of Local Patterns}
\label{ssec:exp2}

The patch-level classification of Gleason grades is performed using the self-learning CNN model detailed in Section \ref{ssec:meth1} and \ref{ssec:meth2}. 

First, Teacher model is trained during $30$ epochs using SGD optimizer. The learning rate ($\eta$) is initialized to $1\cdot10^{-2}$. After half the iterations, this value decreased in a factor of $10$, and an exponential decay was applied during the last $5$ epochs to stabilize the weights such that: $\eta = 1\cdot10^{-3}\cdot e^{-0.1\cdot t}$, where $t$ is the epoch number. Then, the Gleason grades of all the patches from the training set are inferred, and the label distillation process is performed to obtain a pseudo-supervised dataset. Using this data, Student model is trained during the same number of epochs, and under the same optimizer, and learning rate schedule as the training process of Teacher model. %Then, Student becomes Teacher model, and this process is repeated $T=3$ times.

The figures of merit obtained using the initial Teacher model and the last Student model on the different external datasets are presented in Table \ref{tab:resGleasonGrading}. The confusion matrices of the obtained results are illustrated in Fig. \ref{fig:cm2}.

In order to compare our results with other approaches, a model similar to the one proposed in \cite{Campanella2019Clinical-gradeImages} for MIL classification is implemented. This method, hereafter called $Global-Assignment$, consist in assigning the global label to each patch of the whole slide image, and training a CNN using this pseudo-supervised dataset. We trained a model using the same architecture, optimizer and learning rate schedule than with our proposed Student model following this pseudo-labeling procedure. In order to reduce noise during this process, only slides with one unique Gleason grade were used during training. The obtained results are presented in Table \ref{tab:resGleasonGrading}. Also, the results obtained in \cite{Silva-rodriguez2020GoingR} using supervised models are presented.

% Table with metrics:
\begin{table*}[htb]

    \centering
    \caption{Results for the patch-level Gleason grades classification performed by the different approaches on the different test cohorts. The metrics presented are the accuracy (ACC), the F1-Score (F1S), computed per class and its average, and the Cohen's quadratic kappa ($\kappa$).}
    \label{tab:resGleasonGrading}

    \begin{tabular}{|l|c|ccccc|c|}

    \hline
    \multicolumn{1}{|c|}{\textbf{Method}} & \textbf{ACC} & \multicolumn{5}{|c|}{\textbf{F1S}} & \textbf{$\kappa$}\\
     & & NC & GG3 & GG4 & GG5 & Avg. & \\
    \hline
    \hline
    \multicolumn{8}{c}{SICAP} \\
    \hline
    \hline
    $Supervised$ \cite{Silva-rodriguez2020GoingR} & $0.67$ & $0.86$ & $0.59$ & $0.54$ & $0.61$ & $0.65$ & $0.77$\\
    \hline    
    $Global-Assignement$ & $0.5056$  & $0.0756$  & $0.4408$  & $0.7441$  & $0.0952$ & $0.3389$ & $0.4659$ \\
    \hline
    Teacher-CNN & $0.7229$ & $0.7884$ & $0.6426$ & $0.6426$ & $0.2173$ & $0.6047$ & $0.6360$ \\
    \hline
    Student-CNN & $\mathbf{0.7978}$ & $\mathbf{0.9014}$ & $\mathbf{0.7144}$ & $\mathbf{0.7988}$ & $\mathbf{0.6018}$ & $\mathbf{0.7541}$ & $\mathbf{0.8303}$ \\
    \hline
    \hline
    \multicolumn{8}{c}{ARVANITI} \\
    \hline
    \hline
    $Supervised$ \cite{Silva-rodriguez2020GoingR} & $0.5861$ & $0.566$ & $0.6858$ & $0.4699$ & $0.5603$ & $0.5702$ & $0.641$\\
    \hline    
    $Global-Assignement$ & $0.5547$  & $0.0172$  & $0.6747$  & $0.6120$  & $0.2051$ & $0.3772$ & $0.5012$ \\
    \hline
    Teacher-CNN & $0.7055$ & $0.7266$ & $0.7308$ & $0.6827$ & $0.6666$ & $0.7017$ & $0.7567$ \\
    \hline
    Student-CNN & $\mathbf{0.7226}$ & $\mathbf{0.8366}$ & $\mathbf{0.7653}$ & $\mathbf{0.6230}$ & $\mathbf{0.7029}$ & $\mathbf{0.7319}$ & $\mathbf{0.7930}$ \\
    \hline
    \hline
    \multicolumn{8}{c}{GERYTCH} \\
    \hline
    \hline
    $Supervised$ \cite{Silva-rodriguez2020GoingR} & $0.5136$ & $0.2901$ & $0.6162$ & $0.499$ & $0.4959$ & $0.4753$ & $0.5116$\\
    \hline    
    $Global-Assignement$ & $0.5056$  & $0.0756$  & $0.4408$  & $0.7441$  & $0.0952$ & $0.3389$ & $0.4659$ \\
    \hline
    Teacher-CNN & $0.7893$ & $0.6976$ & $0.7958$ & $0.8356$ & $0.6666$ & $0.7489$ & $0.6943$ \\
    \hline
    Student-CNN & $\mathbf{0.8305}$ & $\mathbf{0.8115}$ & $\mathbf{0.8210}$ & $\mathbf{0.8483}$ & $\mathbf{0.8000}$ & $\mathbf{0.8202}$ & $\mathbf{0.8264}$ \\
    \hline
    
    \end{tabular}

\end{table*}

% Confusion matrices:
\begin{figure*}[htb]
\captionsetup[subfloat]{farskip=1pt,captionskip=0.8pt}
    \begin{center}
    
      \subfloat[\label{fig:cm2a}]{\includegraphics[width=.32\linewidth]{Figures/confusion_matrices/cm_ggrade_student_sicap.jpg}}
      \hspace*{\fill}
      \subfloat[\label{fig:cm2b}]{\includegraphics[width=.32\linewidth]{Figures/confusion_matrices/cm_ggrade_student_arvaniti.jpg}}
      \hspace*{\fill}
      \subfloat[\label{fig:cm2c}]{\includegraphics[width=.32\linewidth]{Figures/confusion_matrices/cm_ggrade_student_gerytch.jpg}}
      \hspace*{\fill}
      
    \caption{Confusion Matrix of the patch-level Gleason grades prediction done by Student CNN on the different test cohorts. (a): SICAP; (b): ARVANITI; (c): GERYTCH.}
    \label{fig:cm2}
    \end{center}
\end{figure*}

The self-learning CNN pipeline (average $\kappa = 0.81$ for Student model) outperformed $Global-Assignement$ method (average $\kappa = 0.47$). Our proposed framework does not introduce noise during the pseudo-labeling process, while $Global-Assignement$ assigns cancerous class to non-cancerous patches. Teacher model reached an inter-database average $\kappa$ of $0.69$, and high precision for the detection of cancerous patterns (inter-database average precision of $0.92$). The slide-level max pooling operation in Teacher model architecture produces backpropagation of the weights for only cancerous patterns that the model classifies with high confidence. Although this phenomenon increases the number of false negative classification for cancerous classes, these samples are discarded during the label-refinement process (see Section \ref{ssec:meth2}). Thus, the obtained pseudo-supervised dataset has low amount of noisy labels, and the Student model reaches an average $\kappa$ of $0.81$ and an average $F1S$ of $0.77$.

Regarding the $Supervised$ model developed in \cite{Silva-rodriguez2020GoingR}, using a CNN trained with annotated patches from SICAP database, a drop in $\kappa$ metric was observed from SICAP test subset ($\kappa = 0.77$) to ARVANITI ($\kappa = 0.64$) and GERYTCH ($\kappa = 0.51$) subsets. In contrast, our weakly-supervised model obtained similar results in the three external dataset: $\kappa = 0.83$ on SICAP, $\kappa = 0.79$ on ARVANITI and $\kappa = 0.82$ on GERYTCH. The proposed weakly supervised pipeline outperforms the methodology presented in \cite{Silva-rodriguez2020GoingR} showing a higher generalization ability. This could be produced by the bias of the annotator produced in supervised learning, which is not present while using global-labels in our pipeline, and the difficulty of obtaining large annotated datasets with heterogeneous patterns.

% --------------------------------
%% Global gleason scoring


\subsection{Biopsy-Level Scoring}
\label{ssec:exp3}

The global scoring of biopsies was carried out using the features extracted by Student model as detailed in Section \ref{ssec:meth3}. The models were trained using the train subset of PANDA dataset for predicting both Gleason score and Grade Group. For the multi-layer perceptron model ($MLP$) Adam was applied as optimizer, using a learning rate of $1\cdot10^{-2}$ during $20$ epochs. Also, the k-Nearest Neighbors was fitted using a $k = 20$, optimized on the validation set of PANDA dataset. The global score of the whole slide images from the test subset of PANDA and SICAP datasets was predicted using both models. The figures of merit are reported in Table \ref{tab:resGleasonScoring}. Also, the confusion matrices of the Grade Group predictions using Student model as feature extractor are illustrated in Fig. \ref{fig:cm3}.

In order to compare our proposed approach with previous state-of-the-art methods, the global score is predicted also using the percentage of each cancerous grade in the tissue. The percentage for certain whole slide image $b$ was obtained from the patch-level predictions $\tilde{y}^{s}_{b,i}$ such that: $perc_{b} = \frac{1}{I} \sum_{i} \tilde{y}^{s}_{b,i}$. Then, two different models were trained to predict Gleason score and Grade Group: $kNN$ as proposed in \cite{Nagpal2019DevelopmentCancer}, using $k=5$, and $MLP$ as proposed in \cite{Silva-rodriguez2020GoingR}. The obtained results in PANDA and SICAP datasets are presented in Table \ref{tab:resGleasonScoring}.


% Table with metrics:
\begin{table}[htb]

    \centering
    \caption{Results of the biopsy-level Gleason scoring in the test subsets. The metric presented is the Cohen's quadratic kappa ($\kappa$).}
    \label{tab:resGleasonScoring}

    \begin{tabular}{|l|c|c|}

    \hline
    \multicolumn{1}{|c|}{\textbf{Method}} & \textbf{Gleason Score} & \textbf{Grade Group}\\
    \hline
    \hline
    \multicolumn{3}{c}{PANDA} \\
    \hline
    \hline
    GG\% + kNN & $0.7936$ & $0.8152$ \\
    \hline
    GG\% + MLP & $\mathbf{0.8054}$   & $0.8229$  \\
    \hline
    Student Features + kNN & $0.7773$ &
    $0.7927$  \\
    \hline
    Student Features + MLP & $0.7954$  & $\mathbf{0.8245}$ \\
    \hline
    \hline
    \multicolumn{3}{c}{SICAP} \\
    \hline
    \hline
    Supervised \cite{Silva-rodriguez2020GoingR} & $0.8177$ & $-$ \\ 
    \hline
    GG\% + kNN & $0.5942$ & $0.5221$  \\
    \hline
    GG\% + MLP &  $0.4861$ & $0.5082$ \\
    \hline
    Student Features + kNN & $\mathbf{0.8299}$ &
    $\mathbf{0.8854}$  \\
    \hline
    Student Features + MLP & $0.3847$  & $0.4421$ \\
    \hline

    
    \end{tabular}

\end{table}

% Confusion matrices:
\begin{figure}[htb]
\captionsetup[subfloat]{farskip=1pt,captionskip=0.8pt}
    \begin{center}
    
      \subfloat[\label{fig:cm3a}]{\includegraphics[width=.45\linewidth]{Figures/confusion_matrices/cm_isup_panda.jpg}}
      \hspace*{\fill}
      \subfloat[\label{fig:cm3b}]{\includegraphics[width=.45\linewidth]{Figures/confusion_matrices/cm_isup_SICAP.jpg}}
      \hspace*{\fill}
      
    \caption{Confusion Matrix of the biopsy-level Grade Group prediction done by the attention-based aggregation using Student CNN as backbone, on the two test cohorts. (a): PANDA; (b): SICAP}
    \label{fig:cm3}
    \end{center}
\end{figure}

Our proposed model based on aggregating patch-level features and $kNN$ classifier outperformed previously state-of-the-art methods based on the use of the percentage of each Gleason grade in the tissue, reaching an average $\kappa$ of $0.84$ for both datasets. Although the results were similar for all models when testing on biopsies from the same center as in the training cohort (PANDA), the performance of neural-networks-based methods dropped on the external dataset (SICAP). The classification stage on neural networks showed overfitting to the training set characteristics in both Gleason grade percentage calculation (based on patch-level classification) and in the global score prediction using the Student model features. The non-parametric use of raw features and $kNN$ generalized better on external datasets. The obtained results are promising, being most of the errors between adjacent classes. Moreover, the model differentiated well critical cases such Grade Group $2$ and $3$, which main difference is only the balance between Gleason grade $3$ and $4$ in the tissue (see Fig. \ref{fig:cm3}). 

%Finally, better results are obtained using Student model (average $\kappa$ of $0.86$ for both datasets) than using Teacher model (average $\kappa$ of $0.80$ for both datasets). This result reinforces the importance of obtaining good localization of Gleason grades in the tissue. A better model characterizing local patches also provides a better representation of the whole slide image and thus a better global scoring.

Representative examples of the obtained results using the CAD system on the external SICAP dataset are presented in Fig. \ref{fig:slides}. The pixel-level heatmaps are obtained by bilinearly interpolating the patch-level predicted probabilities of the closest patches in terms of euclidean distance. Then, the class with highest probability is assigned to each pixel. This figure is organized as follows: each row constitutes a case, and the Gleason grades in the tissue are highlighted in different colors. Also, the Grade Group predicted and the ground truth are indicated. 


\begin{figure*}
    \centering
    
    \renewcommand{\thesubfigure}{a}
    \subfloat[\label{regiona}]{\resizebox{1\textwidth}{!}{
    \begin{tikzpicture}[spy using outlines={circle,yellow,magnification=2,size=3cm, connect spies}]
    \node {\pgfimage[interpolate=true,height=5cm]{Figures/slides/16B0022610_predictions.jpg}};
    \spy on (11.5,0.3) in node [left] at (10,2.5);
    \end{tikzpicture}}}

    \renewcommand{\thesubfigure}{b}
    \subfloat[\label{regionb}]{\resizebox{1\textwidth}{!}{
    \begin{tikzpicture}[spy using outlines={circle,yellow,magnification=4,size=3cm, connect spies}]
    \node {\pgfimage[interpolate=true,height=5cm]{Figures/slides/16B0022612_predictions.jpg}};
    \spy on (-0.4,-1.4) in node [left] at (6,1.5);
    \spy on (11.5,-1) in node [left] at (10,1.5);
    \spy on (-5,0) in node [left] at (2,1.5);
    \end{tikzpicture}}}


    \renewcommand{\thesubfigure}{c}
    \subfloat[\label{regionc}]{\resizebox{1\textwidth}{!}{
    \begin{tikzpicture}[spy using outlines={circle,yellow,magnification=2,size=2cm, connect spies}]
    \node {\pgfimage[interpolate=true,height=5cm]{Figures/slides/16B0022786_predictions.jpg}};
    \spy on (-5,-1) in node [left] at (-5,2);
    \spy on (-1,-1.5) in node [left] at (-2.5,2);
    \spy on (2,0.5) in node [left] at (0,2);
    \spy on (4.5,1.5) in node [left] at (6,-1.5);
    \end{tikzpicture}}}


    \renewcommand{\thesubfigure}{d}
    \subfloat[\label{regiond}]{\resizebox{1\textwidth}{!}{
    \begin{tikzpicture}[spy using outlines={circle,yellow,magnification=8,size=3cm, connect spies}]
    \node {\pgfimage[interpolate=true,height=5cm]{Figures/slides/16B0006694_predictions.jpg}};
    \spy on (-8.5,-1.5) in node [left] at (-6,1.5);
    \spy on (-1.9,1.25) in node [left] at (0,-1.3);
    \spy on (-0.1,1.5) in node [left] at (4,-1.3);
    \end{tikzpicture}}}


    \caption{Examples of the proposed CAD system based on Self-Learning CNNs performance on the external SICAP dataset. In green: Gleason grade $3$; blue: Gleason grade $4$ and red: Gleason grade $5$. The reference and predicted Grade Group (Reference - Predicted) are: (a): ($2$ - $1$); (b): ($2$ - $2$); (c): ($3$ - $3$); (d): ($5$ - $5$).}
    \label{fig:slides}
\end{figure*}

==> backup/06_Conclusions_Backup.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this work, we have proposed a self-learning CNN framework able to perform both Gleason grading of local cancerous patterns and global scoring of prostate whole slide images using only the global Gleason score during a weakly-supervised training.

Our proposed framework is composed by a novel Teacher model based on max-pooling of patch-level inferences of Gleason grades able to perform local classification of Gleason grade using biopsy-level labels. Based on the output of Teacher model and a label refinement post-processing, we propose the training of a patch-level Student model on a pseudo-supervised dataset. In the experimental stage, we validate the patch-level classification on three different external datasets. Student model reaches an inter-datasets average Cohen's quadratic kappa ($\kappa$) of $0.82$ and an f1-score of $0.80$. Our results outperformed previous works based on supervised learning with pixel-level annotations. Moreover, the results between the different test cohorts were similar, while previous supervised methods experimented a drop in performance when testing on external test images. Our proposed weakly-supervised method generalizes better than supervised methods for local Gleason grading, due to the absence of annotator bias and the capability of being trained on large heterogeneous datasets.  

Then, the features learned by the patch-level trained models were used to predict the global Grade Group via an average aggregation and a linear classification layer. The method was tested on two different datasets, reaching an average $\kappa$ of $0.84$. This method was compared with the main approach in the literature for Grade Group prediction using the percentage of the different Gleason grades in the tissue. Our feature-based model showed to better generalize pathologist scoring biopsies than previous approaches.

The promising results presented in this work represent a significant advance in the literature of prostate histology. Using weakly-supervised learning it is possible to grade local patterns in gigapixel whole slide images outperforming supervised methods which require laborious annotations by expert pathologists. 

Further research will focus on studying and improving the image-normalization process of prostate histology samples to use CAD systems in external datasets, which is a vital step for a successful generalization. Also, the proposed weakly-supervised models will be refined to decrease the number of biopsies required during training. 

